Are You Copying My Model? Protecting the Copyright of Large Language Models for EaaS via Backdoor Watermark

Large language models (LLMs) have demonstrated powerful capabilities in both text understanding and generation. Companies have begun to offer Embedding as a Service (EaaS) based on these LLMs, which can benefit various natural language processing (NLP) tasks for customers. However, previous studies have shown that EaaS is vulnerable to model extraction attacks, which can cause significant losses for the owners of LLMs, as training these models is extremely expensive. To protect the copyright of LLMs for EaaS, we propose an Embedding Watermark method called EmbMarker that implants backdoors on embeddings. Our method selects a group of moderate-frequency words from a general text corpus to form a trigger set, then selects a target embedding as the watermark, and inserts it into the embeddings of texts containing trigger words as the backdoor. The weight of insertion is proportional to the number of trigger words included in the text. This allows the watermark backdoor to be effectively transferred to EaaS-stealer's model for copyright verification while minimizing the adverse impact on the original embeddings' utility. Our extensive experiments on various datasets show that our method can effectively protect the copyright of EaaS models without compromising service quality.

==> src/problem.tex <==
\section{Problem Definition and Threat Model}
% 介绍EaaS输入输出
\subsection{Problem Definition}


\Subsection{Threat Model}
\subsection{Adversary's Goal}
Like the previous works of model extraction attacks \cite{krishna2019thieves, zanella2020analyzing, he2021model, liu2022stolenencoder}, we consider that an adversary's objective is to steal the embedding of the victim model via continuous query black-box API on cloud EaaS platform, and use these embedding as traning data to develop a model with similar functions.\par
Specifically, Suppose a victim model $V$, which is encapsulated in the cloud API of EaaS platform and can generate embeddings $e$ for various downstream tasks. The adversary can craft text dataset $T$ from a public corpus and query the API with $T$ to obtain embeddings of the victim model. The adversary can craft text $T$ from a public corpus and query the API with $T$ to obtain embeddings of the victim model. Then, the adversary uses stolen embeddings to train a similar model that could provide the same service. It is worth noting that the services provided by the adversary‘s model can be sold at a lower price, since their stealing cost is much lower than training a model from scratch. 
\subsection{Adversary's Capacity}
We assume the adversary have a off-the-shelf PTM such as bert, roberta, etc, and can access the API for unlimited times, which means the adversary can obtain the embeddings of whole text dataset $T$. For example, if a adversary want to steal a model for news embedding generation, the adversary have sufficient budget to continuous query the API until all news embedding obtained. 
\subsection{Adversary's Knowledge}
The model contained in the API is a black box for the adversary, so the adversary is unaware of the structure, corresponding training data, and underlying workings of the victim model. However, the adversary will be aware that the victim model contains a watermark. Therefore, the attacker might employ some methods to detect or eliminate watermarks. 
\subsection{EaaS provider's Goal}
Similar to the goal of previous watermark studies\cite{uchida2017embedding, MengLi2020ProtectingTI, JianHanLim2020ProtectSA}, we assume that the EaaS provider's goal is to implant a endurable marker on victim model, which should has no noticeable impact on model's performance and can be used to trace copyright infringement.\par
Specifically, Assume a victim model $V$ which can provide EaaS to customers and a watermark function $B(\cdot)$ which can embed a watermark into the embedding $e$ generated by $V$. On the one hand, the EaaS provider needs to ensure that the embedded watermark and the original embedded watermark have similar performance on downstream tasks. On the other hand, if the adversary discloses the stolen model API, the EaaS provider can declare the ownership of the model through specific embedding input $e$ and verification algorithm $P(\cdot)$.
\par

\subsection{EaaS provider's Knowledge}
The EaaS provider have full control of victim model, including its model structure, training data and watermark algorithm. However, EaaS provider knows nothing about the model structure and training data domain of the adversary.
